Learning language variations in news corpora through differential embeddings

There is an increasing interest in the NLP community in capturing variations in the usage of language, either through time (i.e., semantic drift), across regions (as dialects or variants) or in different social contexts (i.e., professional or media technolects). Several successful dynamical embeddings have been proposed that can track semantic change through time. Here we show that a model with a central word representation and a slice-dependent contribution can learn word embeddings from different corpora simultaneously. This model is based on a star-like representation of the slices. We apply it to The New York Times and The Guardian newspapers, and we show that it can capture both temporal dynamics in the yearly slices of each corpus, and language variations between US and UK English in a curated multi-source corpus. We provide an extensive evaluation of this methodology.

==> tikz_nn2_figure.tex <==

\def\layersep{1.8cm}

\newsavebox\mybox
\savebox\mybox{%
\tikz\draw[line width=0.7pt] (-0.2,-0.2)--(-0.05,-0.2)--(0.05,0.2)--(0.2,0.2)
                           (-0.2,0)--(0.2,0);%
}

\definecolor{myI}{rgb}{1,0.5,0}
%\definecolor{myI}{rgb}{0.5,0.5,0.5}
\definecolor{myO}{rgb}{0,0.5,1}
%\definecolor{myO}{rgb}{0.3,0.3,0.3}

\begin{tikzpicture}[shorten >=1pt,->,draw=black!50, node distance=\layersep]
    \tikzset{%
      block/.style    = {draw, rounded corners, thick, rectangle, minimum height = 3em,
        minimum width = 3em},
      sum/.style      = {draw, circle, node distance = 2cm}, % Adder
      dot/.style      = {draw, thick, circle, node distance = 2cm, minimum width = 2em}, % Adder
      input/.style    = {coordinate} % Input
    }
    \def\symbs{{"\tilde{s}","s"}}

    \tikzstyle{line}=[draw]
    \tikzstyle{every pin edge}=[<-,shorten <=1pt]
    \tikzstyle{neuron}=[circle,fill=black!25,minimum size=15pt,inner sep=0pt]
    \tikzstyle{input neuronI}=[neuron, fill=myI, minimum width = 2em];
    \tikzstyle{input neuronO}=[neuron, fill=myO, minimum width = 2em];
    \tikzstyle{LUT}=[block, minimum width= 2.0em, minimum height = 2.5em];
    \tikzstyle{pathI-1}=[line, thick, color=myI];
    \tikzstyle{pathI-2}=[line, thick, color=myO];
    \tikzstyle{annot} = [text width=4em, text centered]

    \foreach \blocki in {0,...,1}
      \node[input neuronI] (I-1-\blocki) at (-4.21*\blocki+2,0) {$w^I_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}$};
    \foreach \blocki in {0,...,1}
      \node[input neuronO] (I-2-\blocki) at (-4.21*\blocki+4,0) {$w^O_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}$};

      \node (puntos) at (0.9,1.8) {...};

      %
      % Draw the hidden layer nodes
      %\foreach \name / \y in {1,...,2}
    \foreach \blocki in {0,...,1}
      \path node[LUT,align=center, text width=1.4cm] (H-1-\blocki) at (-4.21*\blocki+1*2,\layersep) {\footnotesize $common$ LUT};
    \foreach \blocki in {0,...,1}
      \path node[LUT,align=center, text width=1.5cm] (H-2-\blocki) at (-4.21*\blocki+2*2,\layersep) {\footnotesize $\delta_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}$ \\ LUT};
      % Draw the hidden2 layer nodes
    \foreach \blocki in {0,...,1}
      \node[input neuronI] (H2-1-\blocki) at (-4.21*\blocki+2,2*\layersep) {+};
    \foreach \blocki in {0,...,1}
      \node[input neuronO] (H2-2-\blocki) at (-4.21*\blocki+4,2*\layersep) {+};
    % Draw the output layer node
    \foreach \blocki in {0,...,1}
      \node[dot] (O-\blocki) at (-4.21*\blocki+3, 2.7*\layersep) {.};
    \foreach \blocki in {0,...,1}
    % Draw the output2 layer node
      \node[LUT, pin={[pin edge={black, ->}, black]0:$p(w^O_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}|w^I_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult})$}] (O2-\blocki) at (-4.21*\blocki+3,3.5*\layersep) {\usebox\mybox};
      % Connect every node in the input layer with every node in the
    \foreach \blocki in {0,...,1}
      \foreach \source in {1,...,2}
          \foreach \dest in {1,...,2}
              \path[pathI-\source] (I-\source-\blocki) edge (H-\dest-\blocki);

    \foreach \blocki in {0,...,1}
      \draw[pathI-1, ->] (H-1-\blocki) -- node[left] {$v_{w^I_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}}^O$}(H2-1-\blocki);
    \foreach \blocki in {0,...,1}
      \draw[pathI-2, ->] (H-1-\blocki) -- node[right] {$v_{w^O_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}}^O$}(H2-2-\blocki);
    \foreach \blocki in {0,...,1}
      \draw[pathI-1, ->] (H-2-\blocki) -- node[left] {$\delta_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult,w^I_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}}$}(H2-1-\blocki);
    \foreach \blocki in {0,...,1}
      \draw[pathI-2, ->] (H-2-\blocki) -- node[right] {$\delta_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult,w^O_{\pgfmathparse{\symbs[\blocki]}\pgfmathresult}}$}(H2-2-\blocki);
      % Connect every node in the hidden2 layer with the output layer
    \foreach \blocki in {0,...,1}
      \foreach \source in {1,...,2}
          \path[pathI-\source] (H2-\source-\blocki) edge (O-\blocki);
      % Connect output2
    \foreach \blocki in {0,...,1}
      \path[thick] (O-\blocki) edge (O2-\blocki);

\end{tikzpicture}

